Representing Data by a Mixture of Activated Simplices

We present a new model which represents data as a mixture of simplices. Simplices are geometric structures that generalize triangles. We give a simple geometric understanding that allows us to learn a simplicial structure efficiently. Our method requires that the data are unit normalized (and thus lie on the unit sphere). We show that under this restriction, building a model with simplices amounts to constructing a convex hull inside the sphere whose boundary facets is close to the data. We call the boundary facets of the convex hull that are close to the data Activated Simplices. While the total number of bases used to build the simplices is a parameter of the model, the dimensions of the individual activated simplices are learned from the data. Simplices can have different dimensions, which facilitates modeling of inhomogeneous data sources. The simplicial structure is bounded --- this is appropriate for modeling data with constraints, such as human elbows can not bend more than 180 degrees. The simplices are easy to interpret and extremes within the data can be discovered among the vertices. The method provides good reconstruction and regularization. It supports good nearest neighbor classification and it allows realistic generative models to be constructed. It achieves state-of-the-art results on benchmark datasets, including 3D poses and digits.

==> egbib_bib <==
%% Created using Papers on Wed, 04 Jun 2014.
%% http://papersapp.com/papers/
@article{CMU_Dataset,
  title={{CMU} Human Motion Capture DataBase. {Availabel} online at http://mocap.cs.cmu.edu/search.html},
  author={ },
  year={2003},
  publisher={}
}

@article{Brown:1979dj,
author = {Brown, Kevin Q},
title = {{Voronoi diagrams from convex hulls}},
journal = {Information Processing Letters},
year = {1979},
volume = {9},
number = {5},
pages = {223--228},
month = jan
}


@article{Ananymous:2013tw,
author = {{Ananymous}},
title = {{Preconditioning for Accelerated Iteratively Reweighted Least Squares in}},
journal = {CVPR submission},
year = {2013},
pages = {1--8},
month = nov
}

@article{Edelsbrunner:1983fe,
author = {Edelsbrunner, H and Kirkpatrick, D and Seidel, R},
title = {{On the shape of a set of points in the plane}},
journal = {Information Theory, IEEE Transactions on},
year = {1983},
volume = {29},
number = {4},
pages = {551--559}
}

@article{Edelsbrunner:1998wx,
author = {Edelsbrunner, Herbert},
title = {{Shape reconstruction with Delaunay complex}},
year = {1998},
pages = {119--132}
}


@article{Edelsbrunner:1986wt,
author = {Edelsbrunner, Herbert and Seidel, Raimund},
title = {{Voronoi diagrams and arrangements}},
journal = {Discrete {\&} Computational Geometry},
year = {1986},
volume = {1},
number = {1},
pages = {25--44}
}

@inproceedings{Cheng:2005vy,
author = {Cheng, Siu-Wing and Dey, Tamal K and Ramos, Edgar A},
title = {{Manifold reconstruction from point samples}},
booktitle = {SODA '05: Proceedings of the sixteenth annual ACM-SIAM symposium on Discrete algorithms},
year = {2005},
publisher = { Society for Industrial and Applied Mathematics},
month = jan
}


@article{Amenta:1999uj,
author = {Amenta, Nina and Bern, Marshall},
title = {{Surface reconstruction by Voronoi filtering}},
journal = {Discrete {\&} Computational Geometry},
year = {1999},
volume = {22},
number = {4},
pages = {481--504}
}

@inproceedings{Amenta:2000it,
author = {Amenta, N and Choi, S and Dey, T K and Leekha, N},
title = {{A simple algorithm for homeomorphic surface reconstruction}},
booktitle = {SCG '00: Proceedings of the sixteenth annual symposium on Computational geometry},
year = {2000},
pages = {1--10},
publisher = { ACM  Request Permissions},
month = may
}


@article{Edelsbrunner:2003wp,
author = {Edelsbrunner, Herbert},
title = {{Surface reconstruction by wrapping finite sets in space}},
year = {2003},
pages = {379--404}
}

@inproceedings{Dey:2003jf,
author = {Dey, Tamal K and Goswami, Samrat},
title = {{Tight cocone: a water-tight surface reconstructor}},
booktitle = {SM '03: Proceedings of the eighth ACM symposium on Solid modeling and applications},
year = {2003},
publisher = { ACM  Request Permissions},
month = jun
}



@misc{minka2000estimating,
  title={Estimating a Dirichlet distribution},
  author={Minka, Thomas},
  year={2000},
  publisher={Technical report, MIT}
}

@article{ionescu2013human3,
author = {Ionescu, Catalin and Papava, Dragos and Olaru, Vlad and Sminchisescu,  Cristian},
title = {Human3.6M: Large Scale Datasets and Predictive Methods for 3D Human Sensing in Natural Environments},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
publisher = {IEEE Computer Society},
volume = {36},
number = {7},
pages = {1325-1339},
month = {jul},
year = {2014}
}


@article{cutler1994archetypal,
  title={Archetypal analysis},
  author={Cutler, Adele and Breiman, Leo},
  journal={Technometrics},
  volume={36},
  number={4},
  pages={338--347},
  year={1994},
  publisher={Taylor \& Francis}
}

@article{semeion_dataset,
  title = {{Semeion} Handwritten Digit Data Set. http://archive.ics.uci.edu /ml/datasets/Semeion+Handwritten+Digit},
  author={ },
  year={ },
  publisher={}
}

@article{Arthur:2007tv,
author = {Arthur, D and Vassilvitskii, S},
title = {{k-means++: The advantages of careful seeding}},
journal = {Proceedings of the eighteenth annual ACM- {\ldots}},
year = {2007}
}

@article{Baraniuk:2010hg,
author = {Baraniuk, R G and Cevher, V and Duarte, M F and Hegde, C},
title = {{Model-Based Compressive Sensing}},
journal = {Information Theory, IEEE Transactions on},
year = {2010},
volume = {56},
number = {4},
pages = {1982--2001}
}

@article{belhumeur1998set,
author = {Belhumeur, P N and Kriegman, David J},
title = {{What is the set of images of an object under all possible illumination conditions?}},
journal = {IJCV},
year = {1998},
volume = {28},
number = {3},
pages = {245--260}
}

@article{Belkin:2003va,
author = {Belkin, Mikhail and Niyogi, Partha},
title = {{Laplacian eigenmaps for dimensionality reduction and data representation}},
journal = {Neural Computation},
year = {2003},
volume = {15},
number = {6},
pages = {1373--1396}
}

@article{Bradley:2004tz,
author = {Bradley, Efron and Trevor, Hastie and Roberts, T},
title = {{Least angle regression}},
journal = {The Annals of Statistics},
year = {2004},
volume = {32},
number = {2},
pages = {407--499}
}

@article{Bradley:2000cm,
author = {Bradley, P S and Mangasarian, O L},
title = {{k-plane clustering}},
journal = {Journal of Global Optimization.},
year = {2000},
volume = {16},
number = {1},
pages = {23--32}
}

@article{Brand:2003vn,
author = {Brand, Matthew},
title = {{Charting a manifold}},
journal = {NIPS},
year = {2003},
pages = {985--992}
}

@article{Breiman:1995ww,
author = {Breiman, Leo},
title = {{Better subset regression using the nonnegative garrote}},
journal = {Technometrics},
year = {1995},
volume = {37},
number = {4},
pages = {373--384}
}

@article{Canas:2012vf,
author = {Canas, G D and Poggio, Tomaso A and Rosasco, Lorenzo},
title = {{Learning Manifolds with K-Means and K-Flats.}},
journal = {NIPS},
year = {2012}
}

@PhdThesis{Huggins,
           title = "{Sparse Coding via Geometry}",
          author = " Patrick S. Huggins",
          school = "Yale University",
           month = may,
            year = "2005",
}

@article{Candes:2005cs,
author = {Candes, E J and Tao, T},
title = {{Decoding by linear programming}},
journal = {Information Theory, IEEE Transactions on},
year = {2005},
volume = {51},
number = {12},
pages = {4203--4215}
}

@article{Candes:2006eq,
author = {Cand{\`e}s, Emmanuel J and Romberg, Justin and Tao, Terence},
title = {{Robust uncertainty principles: Exact signal reconstruction from highly incomplete frequency information}},
journal = {Information Theory, IEEE Transactions on},
year = {2006},
volume = {52},
number = {2},
pages = {489--509}
}

@article{carlsson2009topology,
author = {Carlsson, Gunnar},
title = {{Topology and data}},
journal = {Bulletin of the American Mathematical Society},
year = {2009},
volume = {46},
number = {2},
pages = {255}
}

@techreport{Carlsson:2003wd,
author = {Carlsson, Gunnar and De Silva, Vin},
title = {{Topological approximation by small simplicial complexes}},
year = {2003}
}

@article{chen1998atomic,
author = {Chen, S S and Donoho, D L and Saunders, M A},
title = {{Atomic decomposition by basis pursuit}},
journal = {SIAM journal on scientific computing},
year = {1998},
volume = {20},
number = {1},
pages = {33--61}
}

@article{Costa:2004gx,
author = {Costa, Jose A and Hero, III, Alfred O},
title = {{Geodesic entropic graphs for dimension and entropy estimation in manifold learning}},
journal = {Signal Processing, IEEE Transactions on},
year = {2004},
volume = {52},
number = {8},
pages = {2210--2221}
}

@article{Donoho:2006ci,
author = {Donoho, D L},
title = {{Compressed sensing}},
journal = {Information Theory, IEEE Transactions on},
year = {2006},
volume = {52},
number = {4},
pages = {1289--1306}
}

@article{Donoho:2009wh,
author = {Donoho, David and Tanner, Jared},
title = {{Counting faces of randomly projected polytopes when the projection radically lowers dimension}},
journal = {Journal of the American Mathematical Society},
year = {2009},
volume = {22},
number = {1},
pages = {1--53}
}

@article{Donoho:2006wk,
author = {Donoho, David L},
title = {{High-dimensional centrally symmetric polytopes with neighborliness proportional to dimension}},
journal = {Discrete {\&} Computational Geometry},
year = {2006},
volume = {35},
number = {4},
pages = {617--652}
}

@techreport{Donoho:2005we,
author = {Donoho, David L},
title = {{Neighborly polytopes and sparse solutions of underdetermined linear equations}},
year = {2005}
}

@article{Donoho:2003tu,
author = {Donoho, David L and Grimes, Carrie},
title = {{Hessian eigenmaps: Locally linear embedding techniques for high-dimensional data}},
journal = {Proceedings of the National Academy of Sciences of the United States of America},
year = {2003},
volume = {100},
number = {10},
pages = {5591--5596}
}

@article{Elhamifar:2013uz,
author = {Elhamifar, E and Vidal, R},
title = {{Sparse subspace clustering: Algorithm, theory, and applications}},
journal = {ieeexplore.ieee.org},
year = {2013}
}

@article{Elhamifar:2010ud,
author = {Elhamifar, E and Vidal, R},
title = {{Clustering disjoint subspaces via sparse representation}},
journal = {Acoustics Speech and Signal Processing {\ldots}},
year = {2010}
}


@article{Friedman:2010uq,
author = {Friedman, J and Hastie, Trevor and Tibshirani, Robert},
title = {{A note on the group lasso and a sparse group lasso}},
journal = {arXiv.org},
year = {2010},
eprint = {1001.0736v1},
eprinttype = {arxiv},
eprintclass = {math.ST},
month = jan
}

@article{Fukunaga:1971vk,
author = {Fukunaga, Keinosuke and Olsen, David R},
title = {{An algorithm for finding intrinsic dimensionality of data}},
journal = {Computers, IEEE Transactions on},
year = {1971},
volume = {100},
number = {2},
pages = {176--183}
}

@article{Georghiades:2001tc,
author = {Georghiades, Athinodoros S and Belhumeur, P N and Kriegman, David},
title = {{From few to many: Illumination cone models for face recognition under variable lighting and pose}},
journal = {PAMI},
year = {2001},
volume = {23},
number = {6},
pages = {643--660}
}

@article{Ham:2004ut,
author = {Ham, Jihun and Lee, Daniel D and Mika, Sebastian and Sch{\"o}lkopf, Bernhard},
title = {{A kernel view of the dimensionality reduction of manifolds}},
year = {2004},
pages = {47}
}

@article{Hong:2013wx,
author = {Hong, Yi and Si, Zhangzhang and Hu, Wenze and Zhu, Song Chun and Wu, Ying},
title = {{Unsupervised learning of compositional sparse code for natural image representation}},
journal = {Quarterly of Applied Mathematics},
year = {2013}
}

@article{Huang:2011is,
author = {Huang, Junzhou and Zhang, Tong and Metaxas, Dimitris},
title = {{Learning with structured sparsity}},
journal = {The Journal of Machine Learning Research},
year = {2011},
volume = {12},
pages = {3371--3412}
}

@article{Lee:2005tv,
author = {Lee, Kuang-Chih and Ho, Jeffrey and Kriegman, David},
title = {{Acquiring linear subspaces for face recognition under variable lighting}},
journal = {PAMI},
year = {2005},
volume = {27},
number = {5},
pages = {684--698}
}

@article{Levina:2004tf,
author = {Levina, Elizaveta and Bickel, Peter J},
title = {{Maximum likelihood estimation of intrinsic dimension}},
journal = {Ann Arbor MI},
year = {2004},
volume = {48109},
pages = {1092}
}

@article{Mairal:2009um,
author = {Mairal, Julien and Bach, Francis and Ponce, Jean and Sapiro, Guillermo},
title = {{Online dictionary learning for sparse coding}},
year = {2009},
pages = {689--696}
}

@book{Matouvsek:2002td,
author = {Matouvsek, Jivri},
title = {{Lectures on Discrete Geometry}},
publisher = {Springer},
year = {2002},
volume = {212}
}

@article{olshausen1996emergence,
author = {Olshausen, B A and Field, D J},
title = {{Emergence of simple-cell receptive field properties by learning a sparse code for natural images}},
journal = {Nature},
year = {1996},
volume = {381},
number = {6583},
pages = {607--609}
}

@article{Osborne:2000ha,
author = {Osborne, Michael R and Presnell, Brett and Turlach, Berwin A},
title = {{On the LASSO and its dual}},
journal = {Journal of Computational and Graphical Statistics},
year = {2000},
volume = {9},
number = {2},
pages = {319--337}
}

@inproceedings{Pitelis:2013ik,
author = {Pitelis, N and Russell, C and Agapito, L},
title = {{Learning a Manifold as an Atlas}},
booktitle = {CVPR},
year = {2013},
pages = {1642--1649}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={IEEE}
}


@article{chen2014fast,
  title={Fast and robust archetypal analysis for representation learning},
  author={Chen, Yuansi and Mairal, Julien and Harchaoui, Zaid},
  journal={arXiv preprint arXiv:1405.6472},
  year={2014}
}

@article{Pitelis:2013wg,
author = {Pitelis, Nikolaos and Russell, Chris and Agapito, Lourdes},
title = {{Learning a Manifold as an Atlas Supplementary Material}},
journal = {CVPR},
year = {2013}
}

@book{wright1999numerical,
  title={Numerical optimization},
  author={Wright, SJ and Nocedal, J},
  volume={2},
  year={1999},
  publisher={Springer New York}
}



@book{Rockafellar:ww,
author = {Rockafellar, R Tyrrell},
title = {{Convex analysis}},
publisher = {Princeton university press},
volume = {28}
}

@article{Roweis:2014vy,
author = {Roweis, S T and Saul, L K and Hinton, Geoffrey E},
title = {{Global coordination of local linear models}},
journal = {NIPS},
year = {2014},
pages = {1--8},
month = may
}

@article{Russell:2011vb,
author = {Russell, Chris and Fayad, Jo{\~a}o and Agapito, Lourdes},
title = {{Energy based multiple model fitting for non-rigid structure from motion}},
year = {2011},
pages = {3009--3016}
}

@article{Saul:2003us,
author = {Saul, L K and Roweis, S T},
title = {{Think globally, fit locally: unsupervised learning of low dimensional manifolds}},
journal = {The Journal of Machine Learning Research},
year = {2003}
}

@article{Simon:2013ip,
author = {Simon, Noah and Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
title = {{A Sparse-Group Lasso}},
journal = {Journal of Computational and Graphical Statistics},
year = {2013},
volume = {22},
number = {2},
pages = {231--245},
month = apr
}

@article{tenenbaum2000global,
author = {Tenenbaum, Joshua B and De Silva, Vin and Langford, John C},
title = {{A global geometric framework for nonlinear dimensionality reduction}},
journal = {Science},
year = {2000},
volume = {290},
number = {5500},
pages = {2319--2323}
}

@article{tibshirani1996regression,
author = {Tibshirani, Robert},
title = {{Regression shrinkage and selection via the lasso}},
journal = {Journal of the Royal Statistical Society. Series B. Methodological},
year = {1996},
pages = {267--288}
}

@article{Tibshirani:2013uc,
author = {Tibshirani, Ryan J},
title = {{The lasso problem and uniqueness}},
journal = {Electronic Journal of Statistics},
year = {2013},
volume = {7},
pages = {1456--1490}
}

@article{Wang:vm,
author = {Wang, C and Wang, Y and Lin, Z and Yuille, Alan L and Gao, Wen},
title = {{Robust Estimation of 3D Human Poses from a Single Image}},
journal = {stat.ucla.edu
}
}

@inproceedings{Wang:2013kv,
author = {Wang, Chunyu and Wang, Yizhou and Yuille, Alan L},
title = {{An Approach to Pose-Based Action Recognition}},
booktitle = {CVPR},
year = {2013},
pages = {915--922}
}

@inproceedings{Wang:2014kv,
author = {Wang, Chunyu and Wang, Yizhou and Lin, Zhouchen and Yuille, Alan L and Gao, Wen},
title = {{Robust Estimation of 3D Human Poses from a Single Image}},
booktitle = {CVPR},
year = {2014},
pages = {}
}

@article{Wang:2004uo,
author = {Wang, Jing and Zhang, Zhenyue and Zha, Hongyuan},
title = {{Adaptive Manifold Learning.}},
year = {2004},
volume = {2004}
}

@article{wu2010learning,
author = {Wu, Ying Nian and Si, Zhangzhang and Gong, H and Zhu, Song Chun},
title = {{Learning active basis model for object detection and recognition}},
journal = {IJCV},
year = {2010},
volume = {90},
number = {2},
pages = {198--235}
}

@article{Zhang:2004ht,
author = {Zhang, Zhenyue and Zha, Hongyuan},
title = {{Principal Manifolds and Nonlinear Dimensionality Reduction via Tangent Space Alignment}},
journal = {SIAM journal on scientific computing},
year = {2004},
volume = {26},
number = {1},
pages = {313--338},
month = jan
}

@article{ZhenyueZhang:hm,
author = {Zhenyue Zhang and Jing Wang and Hongyuan Zha},
title = {{Adaptive Manifold Learning}},
journal = {PAMI},
volume = {34},
number = {2},
pages = {253--265}
}

@inproceedings{li2010action,
  title={Action recognition based on a bag of 3d points},
  author={Li, Wanqing and Zhang, Zhengyou and Liu, Zicheng},
  booktitle={(CVPRW), 2010 IEEE Computer Society Conference on},
  pages={9--14},
  year={2010},
  organization={IEEE}
}

@article{chang2011libsvm,
  title={LIBSVM: a library for support vector machines},
  author={Chang, Chih-Chung and Lin, Chih-Jen},
  journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
  volume={2},
  number={3},
  pages={27},
  year={2011},
  publisher={ACM}
}

@inproceedings{yang2012eigenjoints,
  title={Eigenjoints-based action recognition using naive-bayes-nearest-neighbor},
  author={Yang, Xiaodong and Tian, YingLi},
  booktitle={(CVPRW), 2012 IEEE Computer Society Conference on},
  pages={14--19},
  year={2012},
  organization={IEEE}
}

@inproceedings{nister2006scalable,
  title={Scalable recognition with a vocabulary tree},
  author={Nister, David and Stewenius, Henrik},
  booktitle={CVPR},
  volume={2},
  pages={2161--2168},
  year={2006},
  organization={}
}

@inproceedings{xia2012view,
  title={View invariant human action recognition using histograms of 3d joints},
  author={Xia, Lu and Chen, Chia-Chih and Aggarwal, JK},
  booktitle={CVPR},
  pages={20--27},
  year={2012},
  organization={IEEE}
}


@inproceedings{wang2012mining,
  title={Mining actionlet ensemble for action recognition with depth cameras},
  author={Wang, Jiang and Liu, Zicheng and Wu, Ying and Yuan, Junsong},
  booktitle={Computer Vision and Pattern Recognition (CVPR), 2012 IEEE Conference on},
  pages={1290--1297},
  year={2012},
  organization={IEEE}
}


